Detecting Anomalies within Time Series using Local Neural Transformations

We develop a new method to detect anomalies within time series, which is essential in many application domains, reaching from self-driving cars, finance, and marketing to medical diagnosis and epidemiology. The method is based on self-supervised deep learning that has played a key role in facilitating deep anomaly detection on images, where powerful image transformations are available. However, such transformations are widely unavailable for time series. Addressing this, we develop Local Neural Transformations(LNT), a method learning local transformations of time series from data. The method produces an anomaly score for each time step and thus can be used to detect anomalies within time series. We prove in a theoretical analysis that our novel training objective is more suitable for transformation learning than previous deep Anomaly detection(AD) methods. Our experiments demonstrate that LNT can find anomalies in speech segments from the LibriSpeech data set and better detect interruptions to cyber-physical systems than previous work. Visualization of the learned transformations gives insight into the type of transformations that LNT learns.

==> fig/backward_scoring_fig.tex <==
\begin{tikzpicture}
        
    % Color defintions (https://latexcolor.com/)
    \definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
    \definecolor{cerulean}{rgb}{0.0, 0.48, 0.65};
    \definecolor{carrotorange}{rgb}{0.93, 0.57, 0.13}
    
    % z nodes
    \node[fill, cerulean] (zt) {};
    \node[fill, cerulean, left= 5mm of zt] (ztm1) {};
    \node[fill, cerulean, right= 5mm of zt] (ztp1) {};
    \node[fill, cerulean, right= 5mm of ztp1] (ztp2) {};
    \node[fill, cerulean, right= 5mm of ztp2] (ztp3) {};
    
    % autoregressive part
    \node[draw, circle, inner sep=1pt, above= 3mm of zt, minimum size=3mm] (gart) {};
    \node[draw, circle, inner sep=1pt, above= 3mm of ztp1, minimum size=3mm] (gartp1) {};
    \node[draw, circle, inner sep=1pt, above= 3mm of ztp2, minimum size=3mm] (gartp2) {};
    \node[draw, circle, inner sep=1pt, above= 3mm of ztp3, minimum size=3mm] (gartp3) {};
    \node[draw, circle, inner sep=1pt, above= 3mm of ztm1, minimum size=3mm] (gartm1) {};
    
    
    % c nodes
    \node[fill, celadon, above= 3mm of gartp1] (ctp1) {};
    \node[fill, celadon, above= 3mm of gartp2] (ctp2) {};
    \node[fill, celadon, above= 3mm of gartp3] (ctp3) {};
    \node[fill, celadon, above= 3mm of gart] (ct) {};
    \node[fill, celadon, above= 3mm of gartm1] (ctm1) {};
    
    % Labels
    \node[below= 0 of zt, fill= white, rounded corners, inner sep= 1pt] (lzt) {$z_t$};
    \node[below= 0 of ztm1, fill= white, rounded corners, inner sep= 1pt] (lztm1) {$z_{t-1}$};
    \node[below= 0 of ztp1, fill= yellow, rounded corners, inner sep= 1pt] (lztp1) {$z_{t+1}$};
    \node[below= 0 of ztp2, fill= yellow, rounded corners, inner sep= 1pt] (lztp2) {$z_{t+2}$};
    \node[below= 0 of ztp3, fill= yellow, rounded corners, inner sep= 1pt] (lztp3) {$z_{t+3}$};
    
    \node[above= 0 of ct, fill= yellow, rounded corners, inner sep= 1pt, minimum width= 6mm] (lct) {$c_t$};
    \node[above= 0 of ctp1, fill= white, rounded corners, inner sep= 1pt] (lctp1) {$c_{t+1}$};
    \node[above= 0 of ctp2, fill= white, rounded corners, inner sep= 1pt] (lctp2) {$c_{t+2}$};
    \node[above= 0 of ctp3, fill= white, rounded corners, inner sep= 1pt] (lctp3) {$c_{t+3}$};
    \node[above= 0 of ctm1, fill= white, rounded corners, inner sep= 1pt] (lctm1) {$c_{t-1}$};
    
    % arrows
    \draw[->, black, thick] (zt) -- (gart);
    \draw[->, black, thick] (ztp1) -- (gartp1);
    \draw[->, black, thick] (ztp2) -- (gartp2);
    \draw[->, black, thick] (ztp3) -- (gartp3);
    \draw[->, black, thick] (ztm1) -- (gartm1);
    
    \draw[->, black, thick] (gart) -- (ct);
    \draw[->, black, thick] (gartp1) -- (ctp1);
    \draw[->, black, thick] (gartp2) -- (ctp2);
    \draw[->, black, thick] (gartp3) -- (ctp3);
    \draw[->, black, thick] (gartm1) -- (ctm1);
    
    \draw[->, black, thick] (gart) -- (gartp1);
    \draw[->, black, thick] (gartp1) -- (gartp2);
    \draw[->, black, thick] (gartp2) -- (gartp3);
    \draw[->, black, thick] (gartm1) -- (gart);
    
    % score markers
    \draw[<->, ultra thick, yellow] (lct) to [in=90, out=315] (lztp1);
    \draw[<->, ultra thick, yellow] (lct) to [in=90, out=315] (lztp2);
    \draw[<->, ultra thick, yellow] (lct) to [in=90, out=315] (lztp3);
    
\end{tikzpicture}

==> fig/forward_scoring_fig.tex <==
\begin{tikzpicture}
        
    % Color defintions (https://latexcolor.com/)
    \definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
    \definecolor{cerulean}{rgb}{0.0, 0.48, 0.65};
    \definecolor{carrotorange}{rgb}{0.93, 0.57, 0.13}
    
    % z nodes
    \node[fill, cerulean] (zt) {};
    \node[fill, cerulean, left= 5mm of zt] (ztm1) {};
    \node[fill, cerulean, left= 5mm of ztm1] (ztm2) {};
    \node[fill, cerulean, left= 5mm of ztm2] (ztm3) {};
    \node[fill, cerulean, right= 5mm of zt] (ztp1) {};
    
    % autoregressive part
    \node[draw, circle, inner sep=1pt, above= 3mm of zt, minimum size=3mm] (gart) {};
    \node[draw, circle, inner sep=1pt, above= 3mm of ztp1, minimum size=3mm] (gartp1) {};
    \node[draw, circle, inner sep=1pt, above= 3mm of ztm1, minimum size=3mm] (gartm1) {};
    \node[draw, circle, inner sep=1pt, above= 3mm of ztm2, minimum size=3mm] (gartm2) {};
    \node[draw, circle, inner sep=1pt, above= 3mm of ztm3, minimum size=3mm] (gartm3) {};
    
    % c nodes
    \node[fill, celadon, above= 3mm of gartp1] (ctp1) {};
    \node[fill, celadon, above= 3mm of gart] (ct) {};
    \node[fill, celadon, above= 3mm of gartm1] (ctm1) {};
    \node[fill, celadon, above= 3mm of gartm2] (ctm2) {};
    \node[fill, celadon, above= 3mm of gartm3] (ctm3) {};
    
    % Labels
    \node[below= 0 of zt, fill= yellow, rounded corners, inner sep= 1pt, minimum width= 6mm] (lzt) {$z_t$};
    \node[below= 0 of ztm1, fill= white, rounded corners, inner sep= 1pt] (lztm1) {$z_{t-1}$};
    \node[below= 0 of ztm2, fill= white, rounded corners, inner sep= 1pt] (lztm2) {$z_{t-2}$};
    \node[below= 0 of ztm3, fill= white, rounded corners, inner sep= 1pt] (lztm3) {$z_{t-3}$};
    \node[below= 0 of ztp1, fill= white, rounded corners, inner sep= 1pt] (lztp1) {$z_{t+1}$};
    
    \node[above= 0 of ct, fill= white, rounded corners, inner sep= 1pt] (lct) {$c_t$};
    \node[above= 0 of ctp1, fill= white, rounded corners, inner sep= 1pt] (lctp1) {$c_{t+1}$};
    \node[above= 0 of ctm1, fill= yellow, rounded corners, inner sep= 1pt] (lctm1) {$c_{t-1}$};
    \node[above= 0 of ctm2, fill= yellow, rounded corners, inner sep= 1pt] (lctm2) {$c_{t-2}$};
    \node[above= 0 of ctm3, fill= yellow, rounded corners, inner sep= 1pt] (lctm3) {$c_{t-3}$};
    
    % arrows
    \draw[->, black, thick] (zt) -- (gart);
    \draw[->, black, thick] (ztp1) -- (gartp1);
    \draw[->, black, thick] (ztm1) -- (gartm1);
    \draw[->, black, thick] (ztm2) -- (gartm2);
    \draw[->, black, thick] (ztm3) -- (gartm3);
    
    \draw[->, black, thick] (gart) -- (ct);
    \draw[->, black, thick] (gartp1) -- (ctp1);
    \draw[->, black, thick] (gartm1) -- (ctm1);
    \draw[->, black, thick] (gartm2) -- (ctm2);
    \draw[->, black, thick] (gartm3) -- (ctm3);
    
    \draw[->, black, thick] (gart) -- (gartp1);
    \draw[->, black, thick] (gartm1) -- (gart);
    \draw[->, black, thick] (gartm2) -- (gartm1);
    \draw[->, black, thick] (gartm3) -- (gartm2);
    
    % score markers
    \draw[<->, ultra thick, yellow] (lctm1) to [in=90, out=315] (lzt);
    \draw[<->, ultra thick, yellow] (lctm2) to [in=120, out=315] (lzt);
    \draw[<->, ultra thick, yellow] (lctm3) to [in=150, out=315] (lzt);
    
\end{tikzpicture}

==> fig/joint_cpc_neutral.tex <==
\begin{tikzpicture}
        
    % Color defintions (https://latexcolor.com/)
    \definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
    \definecolor{cerulean}{rgb}{0.0, 0.48, 0.65};
    \definecolor{carrotorange}{rgb}{0.93, 0.57, 0.13}
    
    % z nodes
    \node[fill, cerulean] (zt) {};
    \node[fill, cerulean, left= of zt] (ztm1) {};
    \node[fill, cerulean, left= of ztm1] (ztm2) {};
    \node[fill, cerulean, right= of zt] (ztp1) {};
    \node[fill, cerulean, right= of ztp1] (ztp2) {};
    \node[fill, cerulean, right= of ztp2] (ztp3) {};
    
    % autoregressive part
    \node[draw, circle, inner sep=1pt, above= 3mm of zt] (gart) {\tiny{RNN}};
    \node[draw, circle, inner sep=1pt, above= 3mm of ztm1] (gartm1) {\tiny{RNN}};
    \node[draw, circle, inner sep=1pt, above= 3mm of ztm2] (gartm2) {\tiny{RNN}};
    
    % c nodes
    \node[fill, celadon, above= 3mm of gart] (ct) {};
    \node[fill, celadon, above= 3mm of gartm1] (ctm1) {};
    \node[fill, celadon, above= 3mm of gartm2] (ctm2) {};
    
    % Labels
    \node[right= 0 of zt]{$z_t$};
    \node[right= 0 of ztm1]{$z_{t-1}$};
    \node[right= 0 of ztm2]{$z_{t-2}$};
    \node[right= 0 of ztp1]{$\cdots$};
    \node[right= 0 of ztp2]{$z_{t+k}$};
    \node[right= 0 of ct, yshift= -2mm]{$c_t$};
    
    % arrows
    \draw[->, black, thick] (zt) -- (gart);
    \draw[->, black, thick] (ztm1) -- (gartm1);
    \draw[->, black, thick] (ztm2) -- (gartm2);
    
    \draw[->, black, thick] (gart) -- (ct);
    \draw[->, black, thick] (gartm1) -- (ctm1);
    \draw[->, black, thick] (gartm2) -- (ctm2);
    
    \draw[->, black, thick] (gartm1) -- (gart);
    \draw[->, black, thick] (gartm2) -- (gartm1);
    
    % encoder
    \node[draw, trapezium, inner sep=2pt, below= 2mm of zt] (genct) {\tiny{encoder}};
    \node[draw, trapezium, inner sep=2pt, below= 2mm of ztm1] (genctm1) {\tiny{encoder}};
    \node[draw, trapezium, inner sep=2pt, below= 2mm of ztm2] (genctm2) {\tiny{encoder}};
    \node[draw, trapezium, inner sep=2pt, below= 2mm of ztp1] (genctp1) {\tiny{encoder}};
    \node[draw, trapezium, inner sep=2pt, below= 2mm of ztp2] (genctp2) {\tiny{encoder}};
    \node[draw, trapezium, inner sep=2pt, below= 2mm of ztp3] (genctp3) {\tiny{encoder}};
    
    % Example Audio Signal
    \node[below= -1mm of genct, xshift=6mm] {\resizebox{\linewidth}{8mm}{\input{img/signal.pgf}}};
    
    % input signal labels
    \node[below= 7mm of genct]{$x_t$};
    \node[below= 7mm of genctm1]{$x_{t-1}$};
    \node[below= 7mm of genctm2]{$x_{t-2}$};
    \node[below= 7mm of genctp1]{$\ldots$};
    \node[below= 7mm of genctp2]{$x_{t+k}$};
    \node[below= 7mm of genctp3]{$\ldots$};
    
    % signal separators
    \draw[-,gray] ($(genct.south east) - (-4.5mm, 0mm)$) -- ($(genct.south east) - (-4.5mm, 10mm)$);
    \draw[-,gray] ($(genctm1.south east) - (-4.5mm, 0mm)$) -- ($(genctm1.south east) - (-4.5mm, 10mm)$);
    \draw[-,gray] ($(genctm2.south east) - (-4.5mm, 0mm)$) -- ($(genctm2.south east) - (-4.5mm, 10mm)$);
    \draw[-,gray] ($(genctp1.south east) - (-4.5mm, 0mm)$) -- ($(genctp1.south east) - (-4.5mm, 10mm)$);
    \draw[-,gray] ($(genctp2.south east) - (-4.5mm, 0mm)$) -- ($(genctp2.south east) - (-4.5mm, 10mm)$);
    
    % Transformed representations
    \node[draw, rounded corners, above= 2mm of ztp2] (neutral) {\small Local Transformations};
    \node[fill, carrotorange, above= 4mm of neutral] (ztl2) {};
    \node[fill, carrotorange, left= 5mm of ztl2] (ztl1) {};
    \node[fill, carrotorange, right= 5mm of ztl2] (ztl3) {};
    \node[fill, carrotorange, above= 8mm of ztl2] (zttilde) {};
    
    \draw[->, dashed, black] (ct) to [in=180, out=0] (zttilde);
    \draw[->, black, thick] (ztp2) -- (neutral);
    \draw[->, black, thick] (neutral) to[in=270, out=90] (ztl1);
    \draw[->, black, thick] (neutral) to[in=270, out=90] (ztl2);
    \draw[->, black, thick] (neutral) to[in=270, out=90] (ztl3);
    
    \node[right= 0mm of zttilde] {$W_k c_t$};
    %\node[left= 0mm of ztl1] {$z_{t+k}^{(1)}$};
    \node[right= 0mm of ztl3] {$z_{t+k}^{(l)}$};
    
    
    % Pushing arrows
    \draw[stealth - stealth, carrotorange] (ztl1) -- (ztl2);
    \draw[stealth - stealth, carrotorange] (ztl2) -- (ztl3);
    \draw[stealth - stealth, carrotorange] (ztl1) to[in=135, out=45] (ztl3);
    % Pulling arrows
    \draw[stealth reversed - stealth reversed, carrotorange] (zttilde) to[in=90, out=270] (ztl1);
    \draw[stealth reversed - stealth reversed, carrotorange] (zttilde) to[in=90, out=270] (ztl2);
    \draw[stealth reversed - stealth reversed, carrotorange] (zttilde) to[in=90, out=270] (ztl3);
    
    % Legend
    \path (current bounding box.north west)
     node[matrix,anchor=north west,cells={nodes={font=\sffamily,anchor=west}},
     draw,inner sep=1mm, xshift=2em, yshift= -0.5em]{
      \draw[stealth - stealth, carrotorange](0,0) -- ++ (0.3,0); & \node{\tiny push}; &
      \draw[stealth reversed - stealth reversed, carrotorange](0,0) -- ++ (0.3,0); & \node{\tiny pull};\\
     };
    
\end{tikzpicture}
